Combined Sampling and Optimization Based Planning for Legged-Wheeled Robots

Planning for legged-wheeled machines is typically done using trajectory optimization because of many degrees of freedom, thus rendering legged-wheeled planners prone to falling prey to bad local minima. We present a combined sampling and optimization-based planning approach that can cope with challenging terrain. The sampling-based stage computes whole-body configurations and contact schedule, which speeds up the optimization convergence. The optimization-based stage ensures that all the system constraints, such as non-holonomic rolling constraints, are satisfied. The evaluations show the importance of good initial guesses for optimization. Furthermore, they suggest that terrain/collision (avoidance) constraints are more challenging than the robot model's constraints. Lastly, we extend the optimization to handle general terrain representations in the form of elevation maps.

==> preprocessing.tex <==
\section{MAP PRE-PROCESSING}
\label{sec::map_preprocessing}
Given the environment's 2.5D elevation map, our approach computes other quantities needed for the algorithm to function correctly. The elevation map can be built from the range sensor data and computed using existing approaches \cite{fankhauser2014robot}. For each position $(x,y)$, we compute the terrain normal vectors, smoothed height estimate, and traversability. Computing the normal vectors and height smoothing is done by fitting a plane at position $(x,y)$  locally in a pre-defined neighborhood. 

We compute a normal in the form $\boldsymbol{n} = [n_x \: n_y \: 1]^T$ and height $h_0$ for each point $\boldsymbol{p}_i = (x_i, y_i)$ inside the grid map. The tangent plane at point $\boldsymbol{p}_i$ is a function of local coordinates $dx =x-\boldsymbol{p}_i^x$ and $dy=y-\boldsymbol{p}_i^y$. It can be expressed implicitly as
%
\begin{align}
\label{eq::local_plane}
    \boldsymbol{n}_i^x dx + \boldsymbol{n}_i^y dy + (h-h_i) = 0, \; (x,y) \in \mathbb{R}^2,
\end{align}
%
where $h_i = h(\boldsymbol{p}_i^x,\boldsymbol{p}_i^y)$ is the height of point $\boldsymbol{p}_i$. Assuming that all the points $\boldsymbol{p}_j$ within radius $R$ from $\boldsymbol{p}_i$ lie on the plane, we can write Eq.~\ref{eq::local_plane} in the matrix notation as:
%
\begin{align}
\label{eq::local_plane_vec}
    [\Delta x \: \Delta y \: -1] \cdot \boldsymbol{\theta} = -h_j, \; \forall j \; s.t. \: ||\boldsymbol{p}_j - \boldsymbol{p}_i||_2 < R
\end{align}
%
where $\Delta x = \boldsymbol{p}_j^x - \boldsymbol{p}_i^x$, $\Delta y = \boldsymbol{p}_j^y - \boldsymbol{p}_i^y$ and $\boldsymbol{\theta}$ is a vector of parameters $\boldsymbol{\theta} =[\boldsymbol{n}_i^x \; \boldsymbol{n}_i^y \; h_i]^T$. We can then assemble the data matrix $\boldsymbol{D} \in \mathbb{R}^{M \times 3}$ and estimate the local normal and height of the terrain by solving the least squares:
%
\begin{align}
\label{eq::least_squares}
    \boldsymbol{\theta}^{*} = (\boldsymbol{D}\boldsymbol{D}^{T})^{-1}\boldsymbol{D}^{T}\boldsymbol{h}
\end{align}
%
To estimate terrain normals, plane fitting operation based on Eq.~\ref{eq::local_plane_vec} and \ref{eq::least_squares} is performed. For computing $\boldsymbol{n}^x_i$ and $\boldsymbol{n}^y_i$ we use the radius $R$ of \SI{0.3}{\meter}. 

Also, we perform another filtering with $R$ being equal to \SI{2.5}{\meter}, which is roughly the robot's footprint radius. \emph{initialization} stage of the planner uses the filtering result to determine good base poses. The filtering result is shown in Fig.~\ref{fig::small_block}.
%
\begin{figure}[tb]
\centering
\subfloat[Raw terrain \label{fig::small_block_no_fileter}]{
       \includegraphics[width=0.48\columnwidth]{figures/small_block_no_filter_cropped.png}}
     \subfloat[Filtered terrain  \label{fig::small_block_filtered}]{
       \includegraphics[width=0.48\columnwidth]{figures/small_block_filtered_cropped.png}
     }
    \caption{\textbf{\textit{Left:}} Elevation map of a block with a height jump. The color gradually changes from blue to white, where blue areas are the lowest. \textbf{\textit{Right:}} Filtered elevation map shown in yellow color. Areas with dark yellow color have the lowest height.}
    \label{fig::small_block}
\end{figure}
%
The idea behind heavy filtering shown in Fig.~\ref{fig::small_block} is to use smoothed terrain for computing base poses. Terrain typically involves discontinuities (e.g., steps), which should not be reflected in the base movement since the base moves above the terrain. On the other hand, smoothed terrain (shown in yellow) is a good approximation for base movement, assuming that it stays at some (roughly) constant height above the smoothed terrain. In addition to computing base poses, we can use smoothed terrain to classify traversability. If the terrain is too steep, i.e., if the roll and pitch angle of the terrain normal are too big, we classify the terrain as untraversable. Furthermore, the height difference between smoothed and unsmoothed elevation can detect slopes and gaps.
%
\begin{comment}
 Result of the traversability estimation algorithm is shown in Fig.~\ref{fig::traversability}; blue color means untraversable terrain while the white color depicts traversable terrain. 
 %
\begin{figure}[tb]
\centering
\subfloat[Block terrain \label{fig::small_block_traversability}]{
       \includegraphics[width=0.48\columnwidth]{figures/block_traversability_cropped.png}}
     \subfloat[Rough terrain  \label{fig::rough_terrain_traversability}]{
       \includegraphics[width=0.48\columnwidth]{figures/rough_terrain_traversability.png}
     }
    \caption{\textbf{\textit{Left:}} Elevation map of a block with a height jump. Blue color presents regions labeled as untraversable. \textbf{\textit{Right:}} Rough terrain with the untraversable areas shown in blue color.}
    \label{fig::traversability}
\end{figure}
\end{comment}
%
%
%
%
%
\begin{comment}
I want to tell a story that terrain may vary a lot. and that the base of the robot should not follow every dip and hill in the terrain. Hence we want to filter this out by smoothing the elevation a bit a retaining a "low frequency" height output.
\end{comment}
%
